Learning to Modulate for Non-coherent MIMO

The deep learning trend has recently impacted a variety of fields, including communication systems, where various approaches have explored the application of neural networks in place of traditional designs. Neural networks flexibly allow for data/simulation-driven optimization, but are often employed as black boxes detached from direct application of domain knowledge. Our work considers learning-based approaches addressing modulation and signal detection design for the non-coherent MIMO channel. We demonstrate that simulation-driven optimization can be performed while entirely avoiding neural networks, yet still perform comparably. Additionally, we show the feasibility of MIMO communications over extremely short coherence windows (i.e., channel coefficient stability period), with as few as two time slots.

==> scratch.tex <==

\section{Signal Constellation Optimization}

\subsection{Notation and Conventions}

We consider the $k$-bit message space $\mathcal{M} := \{1, \ldots, 2^k\}$,
where, of course, each message $\m \in \mathcal{M}$ corresponds to a binary representation in $\m' \in \{0, 1\}^k$.
An encoder is specified by a mapping $f : \mathcal{M} \rightarrow \mathbb{R}^n$, which assigns each message $\m \in \mathcal{M}$ to the point $\x = f(\m)$ in $n$-dimensional real space.
The point $\x \in \mathbb{R}^n$ is then transmitted over an $n$-dimensional channel to produce the received signal $\y \in \mathbb{R}^n$, as governed by a conditional probability law $P_{\Y|\X}$.

A soft-output decoder is specified by a mapping $g : \mathbb{R}^n \rightarrow \mathbb{R}^{|\mathcal{M}|}$, where each element in the output vector corresponds to the confidence score that each particular message in $\mathcal{M}$ was transmitted.
The hard decoding decision is made by taking the index that maximizes the score, i.e., $\hat \m = \arg\max_{i \in \mathcal{M}} g(\y)[i]$.

Alternatively, a bitwise soft-output decoder is given by a mapping $g' : \mathbb{R}^n \rightarrow \mathbb{R}^k$, where each element in the output vector corresponds to the confidence score for each individual bit of the transmitted message (with more negative or positive values indicating confidence toward $0$ or $1$, respectively).
The bitwise hard decoding decision is made by $\hat \m' = \mathbf{1}_{[0, \infty)}(g'(\y))$, where $\mathbf{1}_{[0, \infty)}(\cdot)$ denotes the element-wise application of the step function, yielding the binary representation of the decoded message.

\subsection{Theoretical Problem Formulation}

In principle, the design of the communication system can be posed as an optimization problem,
\begin{align*}
\min_{f \in \mathcal{F}, g \in \mathcal{G}} \mathcal{L}(f,g,P_{\Y|\X}),
\end{align*}
where $\mathcal{L}$ is the desired performance metric (loss function) and $\mathcal{F}$, $\mathcal{G}$ are suitable constraint sets.
In additional to capturing practical limitations for optimization (e.g., $\mathcal{F}$, $\mathcal{G}$ may be restricted to parametric families),
the encoder constraints should also incorporate power constraints, such as by restricting the mean,
$\sum_{\m \in \mathcal{M}} \|f(\m)\|^2 \leq nP |\mathcal{M}|$, or maximum, $\max_{\m \in \mathcal{M}} \|f(\m)\|^2 \leq nP$.
Example performance metrics include the block (message) error rate (BLER) $\Pr[\m \neq \hat \m]$ and the bit error rate (BER) $\frac{1}{k}\sum_{i=1}^k \Pr[\m'[i] \neq \hat \m'[i]]$.
However, to enable practical optimization by gradient descent methods, as described in the next subsection, alternative differentiable loss functions are adopted.

\subsection{Optimization via Stochastic Gradient Descent}

The key to enabling end-to-end optimization methods based on gradient descent is the choice of appropriate loss function and parametric families for the encoder and decoder mappings.
A common approach in the literature is to treat the encoder and decoder pair as an {\em autoencoder}, with each implemented as a neural network.
Further, this is commonly paired with cross-entropy loss as the optimization objective.
The remaining subsections detail these approaches.

\subsection{Encoder Realizations}

A {\em Neural Network Encoder} (NNE) could be realized as a Multi-Layer Perceptron (MLP), which generates an output vector by alternatingly applying affine transformations and element-wise nonlinear operations to an input vector.
Assuming that $k$ is small enough that $O(2^k)$ complexity is manageable, the message $\m$ can be input to the NNE as a one-hot encoded vector of length $2^k$, i.e., the input is all zeroes except for
However, when $O(2^k)$ is manageable, the encoder mapping could instead be realized as a {\em Lookup Table} (LUT), which can be directly parameterized by a real matrix $\W$ of dimensionality $n \times 2^k$.
Applying the LUT is clearly equivalent to the basic linear transformation $\W \m$, with $\m$ encoded as a one-hot column vector, corresponding to a minimalist single-layer MLP with no bias or nonlinearity.
Thus, in the regime of small $k$, adopting a deep MLP architecture to realize an NNE is superfluous, since the LUT is both general and much more parameter efficient.
For this LUT encoder, power constraints can be enforced by first centering (subtracting the mean column from each column) and then scaling the result $\W$, e.g., by $\sqrt{\frac{n 2^k P }{ \|\W\|_2^2}}$ to operate at mean power $P$.

For larger $k$, the prohibitive $O(2^k)$ complexity can be avoided by employing an NNE encoder that takes the binary representation of the message $\m' \in \{0, 1\}^k$ as input.

\subsection{Decoder Realizations}

For a given encoder mapping $f$ and known channel model $P_{\Y|\X}$, the soft-output {\em Maximum Likelihood} (ML) decoder produces the likelihoods of each message $\{P_{\Y|\X = f(\m)}\}_{\m \in \mathcal{M}}$.
The bitwise soft-output ML decoder produces the likelihoods for each bit, $\{P_{\Y|\m'[i]=1}\}_{i=1}^k$.
Of course, since exact ML decoding is not always tractable, approximate decoders.

\subsection{MIMO Decoders Scratch}

for comparison we will also consider the case with {\em receiver-CSI}, where both $\Y$ and $\H$ are available to the receiver

In the case with receiver-CSI, the availability of $\H$ allows for tractable calculation of the exact (but unnormalized) log-likelihoods via
\begin{align} \label{eqn:ML-decoding}
g^*(\Y, \H) := \{ -\|\Y - \H f_\C(\m)\|^2 / (2 \sigma^2) \}_{\m \in \{0, 1\}^k}
\end{align}
%, which does not introduce any additional parameters for the decoder.

An alternative approach is to employ a neural network, $h_\theta : \mathbb{C}^{n \times L} \rightarrow \mathbb{C}^{n \times m}$, to estimate the channel matrix as $\hat{\H} := h_\theta(\Y)$, and then calculate the likelihoods assuming $\hat{\H}$, i.e., output the likelihoods as calculated by
\begin{align} \label{eqn:hybrid-decoding}
g^*(\Y, \hat{\H}) = \{ -\|\Y - h_\theta(\Y) f_\C(\m)\|^2 / (2 \sigma^2) \}_{\m \in \{0, 1\}^k}.
\end{align}

Applying the softmax operation (which exponentiates each element of a vector and then scales the vector such that sum is equal to one) to the output vector of any of the decoders produces a stochastic vector (distribution) over the message set $\{0, 1\}^k$.

In the case of receiver-CSI, where the exact log-likelihoods are calculated by~\eqref{eqn:ML-decoding}, the resultant distribution is exactly the posterior $P_{\m | \Y, \H}$.



For the receiver-CSI case, the optimization is only with respect to the codebook $\C$ (since there are no decoder parameters) and is equivalent to maximizing the mutual information $I(\m; \Y, \H)$, that is,
\begin{align} \label{eqn:ML-objective}
\arg \min_\C \E[ - \log P_{\m | \Y, \H}(\m | \Y, \H) ] = \arg \max_\C I(\m; \Y, \H),
\end{align}
where $P_{\m | \Y, \H}$ is produced by applying the softmax operation to the log-likelihoods calculated by~\eqref{eqn:ML-decoding}.

For both cases given in~\eqref{eqn:NN-objective} and~\eqref{eqn:ML-objective}, 

